Genetic-guided GFlowNets for Sample Efficient Molecular Optimization

The challenge of discovering new molecules with desired properties is crucial in domains like drug discovery and material design. Recent advances in deep learning-based generative methods have shown promise but face the issue of sample efficiency due to the computational expense of evaluating the reward function. This paper proposes a novel algorithm for sample-efficient molecular optimization by distilling a powerful genetic algorithm into deep generative policy using GFlowNets training, the off-policy method for amortized inference. This approach enables the deep generative policy to learn from domain knowledge, which has been explicitly integrated into the genetic algorithm. Our method achieves state-of-the-art performance in the official molecular optimization benchmark, significantly outperforming previous methods. It also demonstrates effectiveness in designing inhibitors against SARS-CoV-2 with substantially fewer reward calls.

==> tables/genetic_gfn_al.tex <==
\begin{tabular}{lcc}
\toprule
 & With Genetic Search & With $\eps$-noisy \\
\midrule
\textbf{AUC Top-1} & 13.997 \footnotesize{$\pm$ 0.337} & 11.954 \footnotesize{$\pm$ 0.190} \\
\textbf{AUC Top-10} & 13.462 \footnotesize{$\pm$ 0.303} & 11.257 \footnotesize{$\pm$ 0.171} \\
\textbf{AUC Top-100} & 12.263 \footnotesize{$\pm$ 0.218} & \phantom{1}9.901 \footnotesize{$\pm$ 0.237} \\
\bottomrule
\end{tabular} 

==> tables/score_div.tex <==
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{4}{c}{Inverse temperature} & \multicolumn{4}{c}{Weight-shift factor} \\
\cmidrule(r){2-5} \cmidrule(r){6-9}
 & $\beta = 5$ & $\beta = 10$ & $\beta = 30$ &  $\beta = 50$ & $k=0.1$  & $k=0.05$ & $k=0.01$ & $k=0.005$   \\
\midrule
% \cmidrule(r){2-5} \cmidrule(r){6-9}
\textbf{AUC Top-1} & 15.247 & 15.385 & 16.248 & \textbf{16.527} & 15.246 & 15.801 & \textbf{16.527} & 16.323 \\
\textbf{AUC Top-10} & 14.597 & 14.735 & 15.815 & \textbf{16.213} & 14.652 & 15.330 & \textbf{16.213} & 16.040 \\
\textbf{AUC Top-100} & 13.116 & 13.348 & 14.943 & \textbf{15.516} & 13.597 & 14.453 & \textbf{15.516} & 15.418 \\
\midrule
\textbf{Diversity} & \textbf{0.670} & 0.663 & 0.528 & 0.432  & \textbf{0.581} & 0.515 & 0.432 & 0.444 \\
\bottomrule
\end{tabular} 

% \begin{tabular}{l|cccc}
% \toprule
% Oracle &  $\beta = 5$ & $\beta = 10$ & $\beta = 30$ &  $\beta = 50$ \\
% \midrule
% \textbf{AUC Top-1} & 15.247 & 15.385 & 16.248 & \textbf{16.527}  \\
% \textbf{AUC Top-10} & 14.597 & 14.735 & 15.815 & \textbf{16.213}  \\
% \textbf{AUC Top-100} & 13.116 & 13.348 & 14.943 & \textbf{15.516}  \\
% \textbf{Diversity} & \textbf{0.670} & 0.663 & 0.528 & 0.432 \\
% \bottomrule
% \end{tabular} 
